Better than Average: Paired Evaluation of NLP Systems

Evaluation in NLP is usually done by comparing the scores of competing systems independently averaged over a common set of test instances. In this work, we question the use of averages for aggregating evaluation scores into a final number used to decide which system is best, since the average, as well as alternatives such as the median, ignores the pairing arising from the fact that systems are evaluated on the same test instances. We illustrate the importance of taking the instance-level pairing of evaluation scores into account and demonstrate, both theoretically and empirically, the advantages of aggregation methods based on pairwise comparisons, such as the Bradley-Terry (BT) model, a mechanism based on the estimated probability that a given system scores better than another on the test set. By re-evaluating 296 real NLP evaluation setups across four tasks and 18 evaluation metrics, we show that the choice of aggregation mechanism matters and yields different conclusions as to which systems are state of the art in about 30% of the setups. To facilitate the adoption of pairwise evaluation, we release a practical tool for performing the full analysis of evaluation scores with the mean, median, BT, and two variants of BT (Elo and TrueSkill), alongside functionality for appropriate statistical testing.

==> 02_general_framework_old.tex <==
\section{The Framework}
\label{sec:gen_framework}

\todo[inline]{SE: Naive question: the evaluation setup we talk about below evaluates which system is best (given a fixed metric $M$). While there are also evaluation setups which evaluate which metric is best (using system-level and segment-level evaluation), right? So, we could talk about the evaluation setup to determine the best system or so.}

\subsection{Terminology}
Typically, a standard evaluation setup consists of 4 elements:\todo{SE: maybe call it the reference-based setup, to distinguish from reference-free? MP: It accounts for reference-free also by setting $y_l = \emptyset$. SE: Wouldn't reference-free be to compare $S(x)$ to $x$, i.e., $y_l=x$?}
\begin{enumerate}
    \item At least two systems to compare: $S$ and a baseline $B$ each with an inherent unobserved strength $\lambda_S$ and $\lambda_B$ that we aim to discover.
    
    \item A test dataset $T = \{(x_l, y_l): l=1, \dots ,n\}$: made of $n$ test instances, where $x_l$ is the input and $y_l$ is the target output.\todo{SE: $y_l$ is the human reference, right?}
    
    \item An evaluation metric $M$ comparing system outputs $S(x_l)$ to target outputs $y_l$. The metric is applied on the outputs of the systems for each test instance, producing the \textbf{evaluation scores}, for $S$: $\mathcal{M}_{STM} = \{M(S(x), y): (x,y) \in T\}$.
    
    \item An aggregation mechanism $\Theta$ to decide whether system $S$ is better than baseline $B$ based on the evaluation scores of the two systems. 
    We note 
    \begin{align*}
        \Theta(S, B | T, M)
        % = \Theta(\{M(S(x_l), y_l)\}, \{M(B(x_l), y_l)\})
        = \Theta(\mathcal{M}_{STM}, \mathcal{M}_{BTM})
    \end{align*} 
    the comparison mechanism between $S$ and $B$ on dataset $T$ with evaluation metric $M$. It outputs its guess about which system is the best (or declares the comparison inconclusive if the difference is not statistically significant).
\end{enumerate}

\todo[inline]{SE:
Some minor comments on mathematical notation  (which is certainly very heterogeneous across people and community). I would write something like: $T=\bigl\{(x_l,y_l)\: :\: l=1,\ldots,n\bigr\}$. I would also write "we denote by X the sum of all ..." rather than "we note X the sum of all" - but maybe these are all different conventions
}

For instance, in summarization, $x_l$ is a source document from the test set and $y_l$ its corresponding reference summary and $M$ can be \cpt{ROUGE} \cite{}. The decision mechanism $\Theta$ is most often based on comparing the arithmetic averages:
\begin{equation}
\label{eq:mean_def}
\begin{split}
    &\Theta(S, B | T, M) \\
    &= \begin{cases}
    S, \ \text{if }\sum\limits_{l} M(S(x_l), y_l) >^{*} \sum\limits_{l} M(B(x_l), y_l)\\
B, \ \text{if } \sum\limits_{l} M(B(x_l), y_l) >^{*} \sum\limits_{l} M(S(x_l), y_l)\\
\text{inconclusive}, \ \text{otherwise}.
\end{cases}
\end{split}
\end{equation}

We use $>^*$ to denote statistically significantly greater according to appropriate test. Thus, deciding that $S$ is better than $B$ if the average score of $S$ is (statistically) significantly better than the average score of $B$.

\xhdr{Consistent evaluation result} The outcome of such an evaluation is said to be \emph{consistent} if it recovers the ordering of systems implied by the inherent strengths of systems: %\todo{SE: do we make this notation up or is it standard terminology? The inherent strengths ($\lambda_S,\lambda_B$) have not been introduced but it is probably still clear here, I would say}
\begin{equation}
    \Theta(S, B | T, M) = S \iff \lambda_S > \lambda_B.
\end{equation}


\xhdr{Probabilistic model}
Generally, the test dataset is assumed to be a representative sample of a larger population of instances on which we expect our systems to be deployed. Thus, $(x_l, y_l)$ can be seen as random variable\todo{SE: I would see $(x_l,y_l)$ as a random draw from some random variable with the given distribution?} following a probability distribution $\mathbb{P}_{Task}$ representative of the task\todo{Wei: maybe go straight to introduce $X_S$ and remove the notations $(x_l,y_l)$ and $\mathbb{P}_{Task}$ if they are not further used later.}.

Then, the evaluation scores obtained by a system $S$ are also seen as random variables $X_S$.
% \begin{equation}
%     F(S, T) = [X^l_S]_{l=1}^n
% \end{equation}
Implicitly, $X_S$ follows some distribution $\mathbb{P}$ that depends on the structure of the task $\mathbb{P}_{Task}$, the choice of evaluation metric $M$ and the strength $\lambda_S$ of the system.

In this work, we put the focus on the aggregation mechanism $\Theta$ and question the ubiquity of arithmetic averages to decide which system is better.
In particular, we ask under what properties of $\mathbb{P}$ does using averages produces a consistent evaluation (ordering of systems consistent with inherent strengths) and investigate two robust alternatives to the mean: the median and paired ranking mechanism: Bradley-Terry \cite{bt_one}.
% In this work, we question the decision mechanism $\Theta$ and the ubiquity of the \emph{average} over test scores to decide whether $S$ is better than $B$. 
% Under what properties of $\mathbb{P}$ does using averages produces a consistent evaluation (ordering of systems consistent with inherent strengths).\todo{SE: analyzing aggregation functions is interesting in mathematics (e.g., power means \url{https://hal.archives-ouvertes.fr/hal-00539028/document}) and economics, e.g., Arrow's theorem}


% Each system $s_i$ has an inherent strength $\lambda_i$ that we aim to discover via evaluation.

% We have a test dataset $\{t_l\}, l \in [1, n]$ made of $n$ test data points. Each test point has a latent parameter $\gamma_l$ representing some relevant properties, e.g., its difficulty.

% We then denote $X^l(i)$ the random variable whose outcome is the score obtained by system $s_i$ on the test point $t_l$ measured by some evaluation metric.\todo{SE: $t_l$ would typically be of the form $(x_l,y_l)$ right?} $X^l(i) \sim F(\lambda_i, \gamma_l, u)$ is a random variable following some unspecified probability distribution function of the strength of the system, the data points and some exogeneous noise $u \sim P_U$. Note that $F$ implicitly models the impact of the chosen evaluation metric. 
% \todo[inline]{SE: to have the reader on-board, I would make an example somewhere here, e.g., $x^l(i)=\text{BLEU}(s_i(x_l),y_l)$}

\subsection{Aggregation mechanisms}

We describe three potential decision mechanisms. In the next sections, we investigate the properties of each mechanism.

\xhdr{Mean}
This is the current standard, the average score over test instances is the estimated strength of the system. In a pair of systems, the one with the highest average is declared to be the strongest. We denote this aggregation mechanism as \cpt{Mean}.
It has been described in Eq.~\eqref{eq:mean_def}. 
\todo{SE: yes, that's it, we wanna estimate the strength of the system and different aggregation function are candidates. Then we check which one is consistent in terms of these preferences. Right? Yes!}

% \begin{equation}
%     \Theta(S) = \frac{1}{n} \sum\limits_l M(S(x_l), y_l).
% \end{equation}
% where $x^l_S$\todo{SE: you mean $S(x_l)$ I assume} are sampled following the distribution of $X_S$ to produce test scores on the studied test set.

% Each system $s_i$ receives its average score on the test set:\todo{SE: is this called segment-level eval?}
% \begin{equation}
%     \mathbb{E}[X^l(i)]
% \end{equation}
% Whose particular realization after $X^l(i)$ have been observed to be $x^l(i)$ are:
% \begin{equation}
%     \hat{\mu}_i = \frac{1}{n} \sum\limits_{l} x^l(i)
% \end{equation}

% Then, we say that system $s_i$ is better than $s_j$ according to average aggregation if:
% \begin{equation}
%     \mathbb{E}[X^l(i)] >  \mathbb{E}[X^l(j)],
% \end{equation}
% or, in practice, after making actual observation on the test set:
% \begin{equation}
%      \hat{\mu}_i >  \hat{\mu}_j,
% \end{equation}

\xhdr{Median}
An important alternative to the mean is the median as it is a robust statistic.\todo{SE: Is this actually used by someone in the reality of evaluation. One could also argue it's a robust statistic, that's why it would be intuitive} In our case, the score of the system $S$ is thus obtained as the median of its scores on the test set. Then, in a pair of systems, the one with the highest median scores is declared the strongest. We denote this aggregation mechanism as \cpt{Median}.

% Each system $s_i$ receives its median score on the test set:
% \begin{equation}
%     \mathbb{M}[X^l(i)]
% \end{equation}
% Whose particular realization after $X^l(i)$ have been observed to be $x^l(i)$ is also estimated by the sample median $\hat{m}_i$.

% Then, we say that system $s_i$ is better than $s_j$ according to average aggregation if:
% \begin{equation}
%     \mathbb{M}[X^l(i)] >  \mathbb{M}[X^l(j)],
% \end{equation}
% or, in practice, after making actual observation on the test set:
% \begin{equation}
%     \hat{m}_i >  \hat{m}_j,
% \end{equation}

\xhdr{Bradley-Terry}
The third \se{option we examine here} 
%and maybe less common option 
is given by the Bradley-Terry (BT) model \cite{bt_one}. In this model, systems do not receive a score independently of the scores of other systems. \se{Instead}, the two systems $S$ and $B$ receive scores $\hat{\lambda}_S$ and $\hat{\lambda}_B$ estimated by solving:
% The difference is that systems do not obtain a score on their own, they obtain a score in comparison with respect to other systems. For now, we restrict ourselves to the case of $2$ systems $s_i$ and $s_j$. Each system receives a score $\lambda_i$ computed to solve:
% \begin{align}
%     \frac{\lambda_i}{\lambda_i + \lambda_j} = \mathbb{P}(s_i > s_j),\\
%     \frac{\lambda_j}{\lambda_i + \lambda_j} = \mathbb{P}(s_j > s_i),
% \end{align}

% After particular observations of $X^l(i) = x^l(i)$ on the test set, the systems receives their estimates $\hat{\lambda}_i$ computed by solving the system of two equations:
\begin{align}
    \frac{\hat{\lambda}_S}{\hat{\lambda}_S + \hat{\lambda}_B} &= f_{S>B}, \\
    \frac{\hat{\lambda}_B}{\hat{\lambda}_S + \hat{\lambda}_B} &= 1 - f_{S>B},
\end{align}
where $f_{i>j}$ is the frequency with which system $s_i$ outperforms system $s_j$ on the test set:\todo{SE: one has two equations and two unknowns (the strengths), so this can be inferred using linear algebra..}
\begin{equation}
    f_{S>B} = \frac{|\{l | M(S(x_l), y_l) > M(B(x_l), y_l)\}|}{n}
\end{equation}


% Then, system $S$ is said to be better than $B$ if:\todo{SE: in the last equivalence the equality sign is wrong)}
% \begin{align}
%     & \hat{\lambda}_S >  \hat{\lambda}_B \\
%     \iff & \frac{\hat{\lambda}_S}{\hat{\lambda}_S + \hat{\lambda}_B} > \frac{\hat{\lambda}_B}{\hat{\lambda}_S + \hat{\lambda}_B} \\
%     \iff &\hat{\mathbb{P}}\left(M(B(x), y) > M(S(x), y) | (x,y) \sim \mathbb{P}_{Task}\right)
% \end{align}

The intuitive interpretation is that $\frac{\hat{\lambda}_S}{\hat{\lambda}_S + \hat{\lambda}_B}$ estimates the probability, on an instance sampled from $\mathbb{P}_{Task}$, that system $S$ performs better than system $B$ as measured by metric $M$. Thus, the system with the highest $\hat{\lambda}$ is declared the strongest. We denote this aggregation mechanism as \cpt{BT}.

When two systems are considered, %the problem $\hat{\lambda}$ 
$\hat{\lambda}$s 
can be computed in closed-form.\todo{SE: check my rewrite}

For $k$ systems, we have to rely on an iterative algorithm (guaranteed to converge in our case).\todo{SE: I replaced $n$ by $k$ since $n$ was already used for the number of instances}
\todo{SE: It would be nice to know more about this iterative algorithm with convergence guarantees, but I reckon that we are short on space also}

While \cpt{BT} is a less common option than mean and median, we'll see \se{below} that it satisfies interesting properties making it a strong and robust alternative.

\section{Comparing assumptions}
The roles played by $S$ and $B$ being symmetrical, we now assume without loss of generality that the system $S$ is better than the baseline $B$, i.e., $\lambda_S > \lambda_B$.  

\begin{proposition}
\label{prop:main_prop}
Suppose $\lambda_S > \lambda_B$, and the evaluation scores of $S$ and $B$ are represented by the random variables $X_S$ and $X_B$. 
\begin{itemize}
    \item \cpt{Mean} consistent $\iff  \mathbb{E}[X_S - X_B] > 0$
    \item \cpt{Median} consistent $\iff \mathbb{M}[X_S] - \mathbb{M}[X_B] > 0$.
    \item \cpt{BT} consistent $\iff \mathbb{M}[X_S - X_B] > 0$,
\end{itemize}
where $\mathbb{M}$ is the median. 
$X_S - X_B$ is a random variable obtained by first sampling a test instance $(x_l, y_l)$ and then computing the difference in evaluation score between $S$ and $B$. It reflects the particular paired structure of the evaluation.
\end{proposition}

Note that while the expectation is linear $\mathbb{E}[X_S - X_B] = \mathbb{E}[X_S] - \mathbb{E}[X_B]$, the median is not: $\mathbb{M}[X_S - X_B] \neq \mathbb{M}[X_S] - \mathbb{M}[X_B]$. The non-linearity of the median is the source of what makes the BT and median methods differ.

\xhdr{Comparison \cpt{mean} and \cpt{median}}
It is widely known that the median is an alternative to the mean robust to outliers. This can be seen here because if both $X_S$ and $X_B$ are non-skewed, $\mathbb{E}[X_S] = \mathbb{M}[X_S]$ and $\mathbb{E}[X_B] = \mathbb{M}[X_B]$ and the \cpt{MEAN} and \cpt{Median} give the same ordering of systems. Otherwise, the presence of outliers may shift the one in one direction or another.\todo{SE: the mean in one dir or another?}

\xhdr{Comparison \cpt{mean} and \cpt{BT}}
For simplicity, we note $A_{S,B} = X_S - X_B$ computed as described in \Propref{prop:main_prop}.\todo{SE: I would rewrite this}

First, consider the case when $A_{S, B}$ is non-skewed: then $\mathbb{E}[X_S - X_B] = \mathbb{E}[A_{S, B}] = \mathbb{M}[A_{S, B}]$ and the \cpt{MEAN} and \cpt{BT} produce the same ordering of systems and they are both consistent if $\mathbb{E}[A_{S,B}] = \mathbb{M}[A_{S,B}] > 0$.
Note that it is possible to have $X_S$ and $X_B$ both perfectly symmetrical (non-skewed) and still $A_{S,B}$ very skewed.

% For example, when $A_{S,B}$ follow a non-skewed distribution: $\mathbb{E}[A_{S,B}] = \mathbb{M}[A_{S,B}]$ and thus mean and BT agree on which system is best and they are both correct if and only if $\mathbb{E}[A_{S,B}] = \mathbb{M}[A_{S,B}] > 0$

However, when the variable $A_{S,B}$ is skewed, its mean and its median are different. Then, there are 3 possible cases:
\begin{enumerate}
    \item[(i)] $\mathbb{M}[A_{S,B}] > 0 > \mathbb{E}[A_{S,B}]$: \cpt{BT} is consistent but not the \cpt{mean}. \cpt{mean} and \cpt{BT} disagree on the ordering of systems.
    \item[(ii)] $\mathbb{E}[A_{S,B}] > 0 > \mathbb{M}[A_{S,B}]$: The \cpt{mean} is consistent but not \cpt{BT}. \cpt{mean} and \cpt{BT} disagree on the ordering of systems.
    \item[(iii)] $\mathbb{E}[A_{S,B}] \neq \mathbb{M}[A_{S,B}]$ but they still have the same sign. \cpt{mean} and \cpt{BT} agree on the ordering of systems.
\end{enumerate}

Choosing an aggregation mechanism between \cpt{BT} and \cpt{mean} boils down to deciding what property of the evaluation setup we believe is more likely. In cases (i) and (iii), \cpt{BT} is either as good as or better than \cpt{MEAN}.
But case (ii) means that for most of the test instances the worse system actually obtains a better score but on data points where the ordering is correct the difference is large enough that the overall average is shifted back to the correct ordering.
It appears that if one really believes that the evaluation setup is likely to be in case (ii), the evaluation is not trustworthy in the first place.\todo{SE: It would mean that the in a minority of cases system S beats system B by a lot and in a majority of cases system B wins, right? This could still be realistic, e.g., when it's really close in 51\% of cases (but still B wins) and in the rest S wins by a large margin, couldn't it? Or do you deem this scenario as entirely untrustworthy?} It would assume that observed scores are inconsistent for the majority of test instances.

% Only the two first cases above are relevant to distinguish between BT and mean. 

% In the first case, for most of the test instances the best system actually obtains a better score (thus BT is consistent) but on the datapoints where the ordering is wrong bias the difference in score is large enough that the overall average is biased to produce the inconsistent ordering.

% In the second case, for most of the test instances the worst system actually obtains a better score (thus BT is inconsistent) but on the datapoints where the ordering is correct the difference is large enough that the overall average is lead to produce consistent ordering.

% It appears that if one really believes that the evaluation setup is likely to be in the second case, then one should even trust its evaluation in the first place. It would assume that the observed scores are inconsistent for the majority of instances.

\xhdr{Comparison \cpt{median} and \cpt{BT}}
Based on \Propref{prop:main_prop}, and since the median is not linear, we know that there exist configurations where \cpt{BT} and \cpt{Median} disagree on the ordering of systems.
Understanding these cases is more subtle than with \cpt{Mean} but reveals an important property of evaluation data that is usually ignored but should probably not be: the paired structure.

\cpt{Median} and \cpt{BT} induce the same ordering of systems when $\mathbb{M}[X_S] - \mathbb{M}[X_B] = \mathbb{M}[X_S - X_B]$. In statistics, this is known as bivariate exchangeability. In the rest of the paper, when this property does not hold, we say that there are bivariate exchangeability issues (BEI).

With BEI, it is possible to observe disagreement between \cpt{Median} and \cpt{BT}. A relevant case for NLP is when one system behaves differently on different types of instances, e.g., beyond strong for some types and bad for some others.

% When the random variables $X_S$ and $X_B$ follow distributions where the median of difference is equal to difference of the median $\mathbb{M}[X_S] - \mathbb{M}[X_B] = \mathbb{M}[X_S - X_B]$, BT and median agree on the ordering of systems. In statistics, when properties hold we say that $X_S$ and $X_B$ are bivariate exchangeable (). This happens, when $X_S$ and $X_B$ have the same shape but differ only by a translation of the mean. For example, $\mathcal{N}(0, 1)$ and $\mathcal{N}(2, 1)$ have the same shape with a $|\delta_{\mu}| = 2$, while $\mathcal{N}(0, 1)$ and $\mathcal{N}(0, 2)$ do not have the same shape.
% The property of $X_S$ and $X_B$ where the median of the difference is equal 

% When the $X_S$ and $X_B$ are not bivariate exchangeable, it is possible to observe disagreement between median and BT. A relevant case to the NLP field is when one system behaves differently for different kind of instances, e.g., the system is good for a type of instance and bad on the other.

For instance, consider the two following evaluation scores:
\begin{table}
        \small
        \centering
        \resizebox{0.75\columnwidth}{!}{
        \begin{tabular}{l|ccccc}
        \toprule

         & test 1 & test 2 & test 3 & test 4 & test 5 \\
        \midrule
        $S$     & 1 & 5 & 10 & 12 & 17 \\
        $V$     & 5 & 10 & 12 & 17 & 1 \\
        $B$     & 2 & 6 & 7 & 13 & 18 \\
        % \midrule
        % \midrule
        % & test 1 & test 2 & test 3 & test 4 & test 5 \\
        % \midrule
        % $A$     & 5 & 10 & 12 & 17 & 1 \\
        % $S$     & 2 & 6 & 7 & 13 & 18 \\
        \bottomrule
        
        \end{tabular}
        }
        % \caption{Sliding Masking Analysis: Percentage of decision changed when masking modified token vs. other tokens. The difference is significant ($p$-value$=2.2\cdot10^{-7}$) for funny but not for serious.}\label{tab:sliding-masking}
\end{table}
System $S$ is worse than $B$ on all instances but one. 
System $V$ is better than $B$ on all instances but one.
But system $S$ and $V$ have the exact same set of scores.\todo{SE: took me a while to get this. This list of scores is different, but the \textbf{set} of scores is the same} So any aggregation method, like \cpt{MEan} or \cpt{Median}, that looks at the list of scores of systems separately cannot identify that $V > B > S$. In particular, the mean and median of $S$ are exactly the same as the mean and median of $B$.\todo{SE: S and v have same independent statistics, not S and B, I think}
However, because \cpt{BT} computes for pairs of systems the number of test instances for which one system is better than the other, it can correctly identify the order of systems.
\todo[inline]{SE: nice analysis. When comparing mean and BT you also pointed out failure cases of BT, but here not?}

% In this first case, system $B$ is worse than system $S$ on all instances but one. Therefore $BT$ will give system $S$ as a clear winner, yet the median of $B$ is 10, while the median of $S$ is 7. In the second case, a very different story is told, system $A$ is better on all instances but one, but the median for both $A$ and $B$ systems are the same. Indeed, the median is only a property of a list of number and ignores the pairing. When the pairing matters, the median and BT give different results.

% However, in practice, the two compared systems are evaluated on the same test instances and thus there is a strong pairing in the data. BT is thus more adapted than median.

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
        \includegraphics[width=\linewidth]{images/pairs_perm_0.pdf}
        % \caption{permuation a}
        % \label{fig:geom_perm_a}
    \end{subfigure}%
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
        \includegraphics[width=\linewidth]{images/pairs_perm_1.pdf}
        % \caption{permuation b}
        % \label{fig:geom_perm_b}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
    \centering
        \includegraphics[width=\linewidth]{images/pairs_perm_3.pdf}
        % \caption{permuation c}
        % \label{fig:geom_perm_c}
    \end{subfigure}
    % \begin{subfigure}[t]{0.24\textwidth}
    % \centering
    %     \includegraphics[width=\linewidth]{images/pairs_perm_4.pdf}
    %     \caption{permuation d}
    %     \label{fig:geom_perm_d}
    % \end{subfigure}
    \caption{These plots represents the distribution of test instances with coordinate given by the scores of the two systems being compared, i.e., the $x$-axis is the score $X_A|(x_l, y_l)$ of system $A$ on some test instance (x_l, y_l) and the $y$-axis is the score $X_B|(x_l, y_l)$ of system $B$ on the same instance. While the $3$ represents very different structure a paint a different picture of the performances of $A$ and $B$, the marginal distribution of scores of $A$ and $B$ remain unchanged in the $3$ plots. From such pair-plot, not only do we see the global structure of the pairing between the random variable $X_A$ and $X_B$ but we can also read off the decision of \cpt{mean}, \cpt{median} and \cpt{BT} with the \textbf{Geometrical criteria}: (i) if the prolongation of the means intersect above the $X_A=X_B$ line, then \cpt{Mean} predicts that $A$ is better and $B$ otherwise, (ii) if the prolongation of the medians intersect above the $X_A=X_B$ line, then \cpt{Median} predicts that $A$ is better and $B$ otherwise, (iii) if there is more mass in the upper-left triangle, then \cpt{BT} predicts that system $A$ is better and $B$ otherwise. In that case, it means that most of the test instances are in the upper-left triangle where $X_A>X_B$. We shaded the half-triangle with most mass in the plots above. We see that in the middle plot \cpt{BT} disagrees with \cpt{Mean} and \cpt{median} as it predicts $B$ is the best. \cpt{Mean} and \cpt{Median} cannot capture the difference between these different setups. We discuss how to generate infinitely many such examples in \Appref{sec:more-pairing}.}
%     \caption{In these plots, the systems have been ordered such that the x-axis corresponds to scores of the worst system $X_W$ and the y-axis to scores of the best system $X_B$ (in this case, we define better by: $\mathbb{P}(X_B > X_W) > \mathbb{P}(X_W > X_B)$). 
%     The plots represent the distribution of test instances with coordinate given by the performance of systems, i.e., $x$ for $X_W$ and $y$ for $X_B$.
%     The diagonal line represents test instances on which $X_B$ and $X_W$ have the same score.
%     The one-dimensional density plot in blue is the score distribution of $X_W$, and in green the score distribution of $X_B$.
%     \textbf{Geometrical criteria:}  The mean is consistent ($\mathbb{E}[X_B] > \mathbb{E}[X_W]$) if the prolongation of the means (solid lines) intersect above the diagonal.
%     Similarly, the median is consistent $\mathbb{M}[X_B] > \mathbb{M}[X_W]$ if the prolongation of the medians (dotted lines) intersect above the diagonal.
%     BT will give the system on the x-axis better if most of the mass of the distribution is above the diagonal, and the other system otherwise. Here, by construct, we put the system with most of the mass on the x-axis.
%     These figures exemplify limitations of aggregation functions that ignore the pairing: many different pairing can give rise to the same marginal score distributions. In this plots: (a)~$X_B$, (b)~$X_W$, (c)~$X_B$, and (d)~$X_W$ have the exact same score distribution and (a)~$X_W$, (b)~$X_B$, (c)~$X_W$, and (d)~$X_B$ also have the exact same distribution. The mean and median, and any aggregation method that ignores the pairing, can only view these as 4 times the same comparison between the same two score distributions, yet the pairing reveals 4 very different pictures of the relative strengths of the two systems. Also, in two cases $\mathbb{P}(X_B > X_W) > \mathbb{P}(X_W > X_B)$ disagrees with the mean and median (b) and (d). We discuss how to generate infinitely many such examples in \Appref{sec:more-pairing}.
% }
    \label{fig:geom_crit}
\end{figure*}
    
% \begin{figure}
%     \centering
%     \begin{subfigure}[t]{0.45 \columnwidth}
%     \centering
%         \includegraphics[width=\linewidth]{images/geometrical_criterion_b.pdf}
%         \caption{Case where the mean, the median and average agree on which system is the best. The mean of the best system and the worst are: , the medians are: .}
%         \label{fig:geom_good}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.45\columnwidth}
%     \centering
%         \includegraphics[width=\linewidth]{images/geometrical_criterion_a.pdf}
%         \caption{Case where the mean and the median disagree with BT. The pairing matters, The mean of the best system and the worst are: , the medians are: .}
%         \label{fig:geom_bad}
%     \end{subfigure}
%     \caption{In these figures, the x-axis corresponds to scores of the worst system and the y-axis to scores of the best system. Each point is one test instance $(x_l, y_l)$ placed in these space based on how well both system performed. The mean is consistent (recovers the correct ordering) if the intersection of both means happen on the upper-left triangle of the space, i.e., mean of the best system is greater than the mean of the worst system. Similarly for the median. BT predicts that the system on the y-axis is best if most of the mass is in the upper-left triangle. These two figures are an example of why looking only at the marginal scores of systems (like mean and median) is insufficient: the system in green in (a) has the exact same marginal as the system in blue (b) and the blue system in (a) has the exact same marginal as the system in green in (b). Yet, the pairing is different and a very different is told which is completely ignored by the mean and the median which are only functions of the marginals.}
%     \label{fig:geom_crit}
%     \end{figure}
    
\subsection{Graphical criterion}
\Figref{fig:geom_crit} summarizes the problem of ignoring pairing.
In these two-dimensional plots, we compare the performance of two systems: the evaluation scores of $W$ (green) on the x-axis and the evaluation scores of $B$ (blue) on the y-axis.\todo{SE: why change from S to W?} Each point in this space is a potential test instance and its coordinate is given by the scores of the two systems.\todo{SE: its coordinate gives the scores of the two systems?} 

We also see the marginal distributions of evaluation scores $X_B$ and $X_W$ from which we can read off the mean and median. When the mean of $X_B$ is greater than the mean of $X_W$, the two extend\todo{SE: extended?} lines representing the means meet on the upper-left triangle (above the line: $X_B = X_W$). And similarly for the median.
But mean and median being only functions of the marginals in such 2D plots completely ignore the pairing. 
In the figure, this is illustrated by having 4 different pairing (i.e., different structure of the evaluation) that still give rise to the exact same two marginal evaluation score distributions. 
\cpt{Mean}, \cpt{Median} and any other function of the evaluation score distribution that ignores the pairing cannot capture such nuances in the evaluation setup.

% This is shown by the fact that the marginals of $X_B$ and $X_W$ are exactly reversed in between (a) and (b) yet the structure in the pairing plot is very different. 

On the contrary, \cpt{BT} is a property of the structure of the 2D plot, it predicts that $X_B$ is better than $X_W$ when there is more mass on the upper-left triangle (above the line $X_B=X_W$).\todo{SE: some grammatical error in the first part of the sentence} 
In \Figref{fig:geom_crit}~(b) and \Figref{fig:geom_crit}~(d), we see two instances where \cpt{BT} disagrees with \cpt{Mean} and \cpt{Median}.

This graphical criterion captures the intuition that \cpt{BT} predicts as best the system that wins on most of the test instances.\todo{SE: In NLP (or ML in general), we could think of the case where the test data contains hard and easy cases. Let's say we have a case where one system is consistently better on the easy cases, but considerably worse on the hard cases. My feeling is that BT gets this wrong when the easy cases are in the majority}

\todo[inline]{SE: (i) Figure 1 has a very long legend, consider shortening it. (ii) In retrospect, the choice of $X$ for the scores may not be ideal, because there is no natural association. One could have used $S$ (or maybe $\sigma$) if $S$ were not already taken.}

% \section{BT vs. Mean vs. Median}
% Consider two systems $s_i$ and $s_j$ such that $\lambda_i > \lambda_j$, i.e., $s_i$ is better than $s_j$.
% When do the average and ELO correctly recover the proper ordering?

% We introduce the random variable $A^l(i,j) = X^l(i) - X^l(j)$ or simply $A^l$ which also follows some distribution $F_A(\lambda_i, \lambda_j, \gamma_l, u)$.
% We can formulate simple criteria for when BT or Mean will recover the true ordering based on properties of $A^l$.

% First, note that when $A^l(i,j) > 0$ we have observed an ordering of systems that is consistent with the true ordering: the observed score of $s_i$ is higher than that of $s_j$.\todo{SE: on test point $l$..}
% For the full dataset, we get the following statements:
% Therefore, the ranking based approach give the correct result if $P(A^l > 0) > 0.5$, i.e., it is more likely to make the good observation than the bad.
% The average gives the good answer if $P(\sum_l A^l > 0) > 0.5$, i.e., it is more likely that after averaging the correct order is respected.

% First, suppose $F_A$ is symmetric around its mean $\mu$, then both average and ELO give the good answer iff $\mu$ > 0.
% Second, if $F_A$ is left skewed it is possible to observe $P(A^l > 0) > 0.5 > P(\sum_l A^l > 0)$, i.e., ELO giving the good answer and the average giving the wrong.
% This corresponds to having few outliers driving the average away.

% We can simply state that:
% \begin{itemize}
%     \item $\mathbb{E}[A^l] > 0 \iff $ Average recovers the correct ordering of systems
%     \item $\mathbb{M}[A^l] > 0 \iff $ BT recovers the correct ordering of systems, where $\mathbb{M}$ is the median\todo{SE: is this obvious?}
%     \item $\mathbb{M}[X^l(i)] - \mathbb{M}[X^l(j)] > 0 \iff $ median recovers the correct ordering of systems.
% \end{itemize}

% \subsection{Mean vs. BT}
% \xhdr{Agreement}
% Whenever the median and the mean of $A^l$ coincide, average and ELO\todo{SE: BT?} agree and both find the correct answer iff  $\mathbb{E}[A^l] = \mathbb{M}[A^l] > 0$.\todo{SE: I don't think we need identity. We need that both are positive, I think}

% \xhdr{Disagreement}
% When they disagree, it is possible to have $\mathbb{M}[A^l] > 0 > \mathbb{E}[A^l]$, which can happen for left-skewed distributions. Left-skewness means that most of data points are observed in correct order but for few outliers data-points that are observed in the wrong order the difference can be large and bias the average towards the wrong answer. 
% \xhdr{Which one to trust when there is a disagreement}
% Note that for right-skewed distributions, we can have the opposite effect: $\mathbb{E}[A^l] > 0. > \mathbb{M}[A^l]$. Right-skewness would mean that most of the data points the observed order is wrong but only for a few outliers ordered correctly the difference can bias the average towards the correct answer. If we believe that our observation might be right-skew than we probably don't trust our evaluation in the first place. Indeed, we would rely on outliers to get the right answer for the average.

% \subsection{Median vs. BT}
% One would be tempted to take the median score of systems on the test data $\mathbb{M}[X^l(i)]$ instead of the mean and not use Bradley-Terry model at all. 
% The difference between Median and BT fundamentally comes from the non-linearity of the median:
% \begin{equation}
%     \mathbb{M}[A^l] \neq \mathbb{M}[X^l(i)] - \mathbb{M}[X^l(j)]
% \end{equation}
% However, the left-hand side governs the failure case of BT, while the right-hand side governs the failure case of Median.
% This distinction does not exists for Mean because the mean is linear: $\mathbb{E}[A^l] = \mathbb{E}[X^l(i)] - \mathbb{E}[X^l(j)]$.

% \xhdr{Agreement}
% When the random variable $X^l(i)$ and $X^l(j)$ have the same shape but differ only by a translation of the mean $\delta_{\mu}$, then Median and BT give the same answer. For example, $\mathcal{N}(0, 1)$ and $\mathcal{N}(2, 1)$ have the same shape with a $|\delta_{\mu}| = 2$, while $\mathcal{N}(0, 1)$ and $\mathcal{N}(0, 2)$ do not have the same shape.

% \xhdr{Disagreement}
% There is no simple characterization of BT vs. Median disagreement case as for the average because the interplay between the two depends on the pairing. 

% \xhdr{Who to trust when disagreement}
% Median ignores the pairing of the data while the BT takes the pairing into account. Given that the data is paired,\todo{SE: you mean they make predictions on the same data points, I assume} the pairing should be ignored except under the assumption of data exchangeability.\todo{SE: should be or should not be?} BT does not need this assumption.


\subsection{Connection with statistical testing}
The discussion we had about the differences between \cpt{Mean}, \cpt{Median}, and \cpt{BT} has interesting parallels in statistical testing.

When comparing two means of two systems over the same test set, the recommended statistical test is the paired t-test \cite{fisher-1935}. We use the paired version because the data is naturally paired. 

When comparing the medians of two systems over the same test set, the associated statistical test would be Mood's median test. But the data is paired and Mood's median test ignores the pairing \cite{wilcoxon_weak}.

The paired alternative to the Mood's median test is the sign test which measures whether the median of the difference is significant. This is what \cpt{BT} is measuring (see \Propref{prop:main_prop}).

In statistical testing, it seems obvious that we should use paired version of tests because the data is naturally paired \cite{rankel-etal-2011-ranking}. But we argued here that we could also consider paired aggregation mechanisms like \cpt{BT}. 
Sometimes Wilcoxon signed-rank test \cite{wilcoxon1945individual} is used as an alternative to the sign test because it has more statistical power \cite{Graham:2015,Owczarzak:2012} median's test but \newcite{wilcoxon_weak} showed that it does not properly accounts for the pairing of data.

\paragraph{Why not use directly the median of difference as the aggregation mechanims?} While it would be possible and certainly useful for comparing systems under paired data and potential outliers, it does not output one score for each systems (see the discussion about the sign test in \newcite{dror-etal-2018-hitchhikers}). \cpt{BT} produces the $\hat{\lambda}$ estimates for each system that are overall consistent with this statistic (see \Propref{prop:main_prop}).


% When we report means of two systems over the test set, the standard associated statistical test that measures whether the difference is significant is the paired t-test. Indeed, we use the paired version because the data is paired. 
% In the presence of outliers this is not recommended!

% Should we report the difference in median, the associated statistical test measuring whether the difference in median is significant is the Mood's median test (sometimes Wilcoxon–Mann–Whitney U two-sample test can be used but it is not valid:https://www.tandfonline.com/doi/full/10.1080/00031305.2017.1305291)  Because the data is paired, this is not recommended!

% However, if take the pairing into account and report the median of differences, the associated statistical test is the signed test (the  Wilcoxon signed-rank test can be used for numerical values).
% While the median of difference is the most recommended statistics for comparing two systems under paired data and potential outliers, it does not output one score for each systems.
% BT produces the $\hat{\lambda}$ estimates consistent with this statistic.

% Therefore, we recommend to use the BT to produce scores for systems and use Wilcoxon signed-rank test to test whether the improvements are significant.

% \subsection{More fundamental reason to switch to BT}
% Looking at the description of the failure cases of Median, Mean, and BT, we believe the assumption that ensure BT works is most natural and reasonable to make.

% However, we are dealing with the random variable $A^l$ which is the difference between the scores obtained by two systems on one test data point. 

% The mean is linear so the mean of $A^l$ is the difference of the mean of $X^l(i)$ and $X^l(j)$, i.e., $\mathbb{E}[A^l] = \mathbb{E}[X^l(i)] - \mathbb{E}[X^l(j)]$. However, the median is not linear
% ($\mathbb{M}[A^l] \neq \mathbb{M}[X^l(i)] - \mathbb{M}[X^l(j)]$)\footnote{\url{https://stats.stackexchange.com/questions/232261/how-can-i-prove-that-the-median-is-a-nonlinear-function}}, thus taking the difference between the median score of systems does not give the median of the variable $A^l$. The principled approach to solve this problem is the MLE estimate of the Bradley-Terry model. 

% \subsection{Testing}
% testing skewness of the real data (http://www.lithoguru.com/scientist/statistics/Lecture13.pdf) 

% testing bivariate exchangeability of real data https://arxiv.org/pdf/2005.06095.pdf, https://www.jstor.org/stable/27919612?seq=6#metadata_info_tab_contents can be done via testing whether the two distributions have the same shape (Kolmogorov smirnoff test after mean centering)

% \subsection{Results from Simulations}
% \begin{itemize}
%     \item Binary case (2 systems to compare)
%     \item N-systems to compare
%     \item Varying strength of skewness
%     \item Varying exogeneous noise ($U$ above)
%     % \item When both ELO and average works, measure which one proposes 
% \end{itemize}


% \subsection{Real Data}
% Redo evaluation of shared-task, benchmarks with ELO instead of Average and see what changes. Would the field be directed in different directions, would different teams have won shared-task\todo{SE: Wei can take this task, I assume}

% \subsection{Discussion: Optimizing for ELO}
% How to change our loss function in order to optimize for ELO instead of average.
